MultiHaystack: Benchmarking Multimodal Retrieval and Reasoning over 40K Images, Videos, and Documents

Multimodal large language models (MLLMs) achieve strong performance on benchmarks that evaluate text, image, or video understanding separately. However, these settings do not assess a critical real-world requirement, which involves retrieving relevant evidence from large, heterogeneous multimodal corpora prior to reasoning. Most existing benchmarks restrict retrieval to small, single-modality candidate sets, substantially simplifying the search space and overstating end-to-end reliability. To address this gap, we introduce MultiHaystack, the first benchmark designed to evaluate both retrieval and reasoning under large-scale, cross-modal conditions. MultiHaystack comprises over 46,000 multimodal retrieval candidates across documents, images, and videos, along with 747 open yet verifiable questions. Each question is grounded in a unique validated evidence item within the retrieval pool, requiring evidence localization across modalities and fine-grained reasoning. In our study, we find that models perform competitively when provided with the corresponding evidence, but their performance drops sharply when required to retrieve that evidence from the full corpus. Additionally, even the strongest retriever, E5-V, achieves only 40.8% Recall@1, while state-of-the-art MLLMs such as GPT-5 experience a significant drop in reasoning accuracy from 80.86% when provided with the corresponding evidence to 51.4% under top-5 retrieval. These results indicate that multimodal retrieval over heterogeneous pools remains a primary bottleneck for MLLMs, positioning MultiHaystack as a valuable testbed that highlights underlying limitations obscured by small-scale evaluations and promotes retrieval-centric advances in multimodal systems.

==> section/rebuttal.tex <==
\section*{Rebuttal}



% \subsection*{Weakness 1}
% Thank you for raising this important concern. We agree that if QA pairs were generated and filtered solely by GPT-4o / Gemini-2.5-Flash, the resulting dataset quality and distribution could inherit these models’ biases and preferences. To mitigate this risk, our data construction pipeline is explicitly designed to be human-in-the-loop at multiple stages (as shown in the paper section 3.3 MultiHaystack Construction):
% \\
% 1. \textbf{Human verification and editing in QA generation.}
% After the initial QA pairs are generated by LLMs, we perform systematic human review and editing. Annotators check whether each question is well-formed and aligned with the task definition, and whether the answer is correct and supported by the given evidence. Samples that are unclear, biased, or misaligned are either corrected or discarded. Consequently, the final QA pairs are not raw LLM outputs, but human-curated instances.

% 2. \textbf{Human-enforced “single supported answer” filtering.}
% In the QA filtering stage, human annotators further ensure that each question has exactly one supported answer within the whole dataset. If a question admits multiple plausible answers in the documents, or if no answer can be reliably located, that question is removed or revised. This step emphasizes document-grounded verifiability and reduces the influence of any particular LLM’s preference on the dataset distribution.

% 3. \textbf{Goal of the contextual answerability filter.}
% The contextual answerability filter is specifically designed to remove questions that an LLM can answer without consulting the provided evidence (e.g., purely from parametric knowledge or common sense). In other words, we intentionally keep questions that require reading the given context, so that the benchmark primarily evaluates retrieval and reasoning over evidence rather than reflecting a particular LLM’s built-in knowledge or stylistic tendencies.

% Taken together, these design choices mean that our data construction process does not simply inherit the biases and preferences of GPT-4o or Gemini-2.5-Flash:
% \\
% 1. Extensive human verification and filtering correct many erroneous or biased LLM outputs.

% 2.The strict “single answer + context-dependent” constraints make the dataset distribution driven mainly by the task specification and annotation guidelines, rather than by any single LLM.

% Therefore, we confirm that the overall quality and reliability of our benchmark remains high.

% \subsection*{Weakness 2}
% We appreciate the reviewer’s comment on the realism of our questions, especially for video frames. The apparent “over-specificity” of some prompts is in fact a deliberate design choice driven by the task formulation.

% In our benchmark, each query is intended to be answerable from \textbf{exactly one} ground file in the corpus, while all other items serve as distractors. To guarantee this \textbf{one-to-one} correspondence, the query needs to be sufficiently specific so that the correct answer \textbf{cannot} also be derived from a distractor video/document.

% For example, in the question

% “What kind of personal item is on the face of the girl who is applying dye to her hair?”

% if we simplify it to a more generic question such as

% “What kind of personal item is on the face of the girl?”,

% then any distractor video that simply contains a girl’s face may be retrieved. In that case, the model can generate a plausible answer based on the distractor video, which may look semantically correct, but it is grounded in the \textbf{wrong} evidence. Consequently, the predicted answer will not match our ground-truth answer associated with the designated ground video and will be counted as incorrect.

% Allowing such ambiguous queries would blur the boundary between \textbf{retrieval errors} (selecting the wrong video/document) and \textbf{reasoning/generation errors} (failing to understand the correct one), which is contrary to the goal of our task. Our objective is to evaluate whether models can perform \textbf{fine-grained cross-modal retrieval and grounding in a large corpus}, not merely produce a vaguely compatible answer from any similar scene.

% Therefore, while some questions may look more specific than casual, real-world queries, this specificity is necessary to enforce a unique grounding video/document for each query and to obtain a clean and interpretable evaluation of cross-modal retrieval performance.

% \subsection*{Weakness 3}
% Thank you for raising the concern that our distractor design might inflate difficulty in an unnatural way. Our goal is in fact the opposite: to construct candidate sets that reflect realistic “confusable but distinguishable” options in multimodal retrieval, rather than to adversarially depress retrieval metrics or optimize the benchmark for failure.

% As detailed in Appendix F.2, we follow a data-driven and reproducible procedure instead of manually cherry-picking extremely hard examples. Specifically:

% 1. We first use CLIP to compute the similarity between each question and its ground-truth positive file, and we aggregate these scores to obtain their empirical distribution.
% 2. We then compute the mean of this distribution and define a principled similarity interval around this mean, which is intended to capture \textbf{typical} rather than extreme levels of matching strength.
% 3. Finally, we select distractor files whose similarity to the query falls within this interval and include them in our dataset.

% This construction ensures that distractors are semantically related enough to be plausible retrieval candidates, inducing realistic near-miss and near-duplicate confusions that users frequently encounter in real-world retrieval scenarios. At the same time, it avoids focusing on pathological edge cases that would be unlikely to arise from authentic user queries. For these reasons, we believe our distractor design does not artificially overstate the difficulty of the task, but instead better aligns the benchmark with real-world multimodal information-seeking behavior.

% \subsection*{Question 1}
% Thank you for raising this question. A “Gold-in-Top-1” case only indicates that the passage containing the gold answer is ranked first, not that the model will necessarily answer correctly. There are two main reasons:

% 1. \textbf{Final QA pairs differ from the original LLM generations}
    
%     As explained in our response to \textbf{Weakness 1}, all candidate QA pairs are carefully human-calibrated and rewritten before inclusion, to ensure clarity and a \textbf{unique} document-supported answer. This introduces a distribution shift, so GPT-5 / Gemini-2.5-Flash at evaluation time are \textbf{not} simply recalling their earlier generations.
    
% 2. \textbf{Models still make errors in reading and reasoning}
    
%     Even with the correct evidence at Top-1, the model must still locate the relevant span, perform possibly compositional reasoning, and produce an exact answer. Current LLMs are imperfect in this stage. Moreover, our evaluation is strict: outputs with format issues or missing/extra critical information are counted as incorrect, which naturally keeps Gold-in-Top-1 accuracy below 100\%.


% \subsection*{Question 2}
% Thank you for the suggestion. We agree with the motivation of using a human-authored subset to calibrate realism and linguistic variety and to further reduce dependence on generative model biases.

% In the current work, we \textbf{do not include a separate subset written entirely from scratch by humans}, but our data curation process is fundamentally \textbf{human-in-the-loop} rather than a direct adoption of LLM outputs. LLMs are only used to propose candidate QA pairs; all items in the final dataset go through strict human review, rewriting, and filtering to ensure natural and clear questions, uniquely supported answers, and to correct potential biases and overly templated patterns. After this process, many QA pairs are effectively very close to “human-authored,” which to a large extent plays the calibration role the reviewer has in mind and mitigates reliance on any single generative model.

% We agree that explicitly adding a labeled \textbf{human-authored subset} would be a valuable extension, but it is not included in this version due to annotation cost. We will highlight this as a limitation and a direction for future work.

\section*{Reviewer MoTo (4)}
We appreciate your positive assessment of our \textbf{writing clarity, effective figures, and rigorous validation and analysis}.
We will address your concern and answer your questions below.

\textbf{W1.~LLM Dependence.}
LLMs are used only to \emph{propose} drafts; the final QA set is shaped by  
(1) strict evidence-verifiability and single-answer constraints,  
(2) cross-model filtering that removes stylistic or preference-driven patterns, and  
(3) human rewriting that enforces explicit grounding anchors.  
These steps decouple the final QA distribution from the initial GPT/Gemini drafts.  
Empirically, the experimental results show no performance advantage for GPT/Gemini-family models, confirming that the benchmark does not encode model-specific biases.

\textbf{W2.~Question Realism.}
Fine-grained cues are necessary because  
(1) each query must map to \emph{exactly one} item in a 46K multimodal pool,  
(2) generic phrasing would make multiple distractors appear plausible, undermining retrieval evaluability, and  
(3) detailed anchors ensure cross-video discrimination rather than within-video search.  
This avoids the ambiguity shown in Fig.~1 and Fig.~B.1.  
Near-duplicate scenes are common in realistic retrieval settings; thus, specificity reflects real-world constraints rather than artificial difficulty.

\textbf{W3.~Distractor Difficulty.}
Distractors come from a principled, data-driven pipeline rather than adversarial design.  
(1) Stage~4 (Sec.~3.3) retrieves semantically related items via keyword+embedding similarity, mirroring realistic retrieval outputs; no hand-crafted hard cases are introduced.  
(2) Large multimodal corpora naturally contain near-miss items (e.g., similar logos/packaging), and our CLIP-based filtering preserves this distribution while human checks ensure none contain the gold evidence.  
(3) Fig.~9 shows smooth degradation from 1K→10K→46K candidates; engineered difficulty would produce discontinuities, which we do not observe.  
(4) Suppressing near-misses would yield an unrealistic retrieval distribution; keeping them maintains natural retrieval difficulty.

\textbf{Q1.~Gold-in-Top-1 Gap.}
Gold-in-Top-1 evaluates retrieval only; models must still extract the answer correctly.  
(1) All QA pairs are human-rewritten under the single-answer constraint, producing a stricter distribution than the initial LLM drafts, so models are not “answering their own generations.”  
(2) Fig.~8 shows post-retrieval errors in span selection, text reading, numerical/chart interpretation, and layout reasoning—even with the gold item at rank~1.  
(3) Many questions depend on small visual/textual cues that must be read from the retrieved file; parametric guessing is insufficient.  
Thus, Gold-in-Top-1 is an upper bound on retrieval, not on grounded QA.

\textbf{Q2.~Human-authored Subset.}
The benchmark targets evidence-grounded retrieval rather than free-form question writing.  
Human rewriting already ensures natural phrasing and unique grounding at scale.  
A fully human-authored subset at 46K scale would make enforcing single-supported-answer constraints prohibitively expensive and risk reintroducing ambiguity.  
We view such a subset as a valuable direction for future versions.



% \subsection*{Weakness 1}
% Our work primarily focuses on constructing and analyzing a large-scale cross-modal benchmark to systematically reveal the limitations of existing models when retrieving across images, videos, and documents, rather than proposing a new retrieval method. We agree that designing methods tailored to this challenging setting is an important next step. Based on the error patterns observed on our benchmark, we plan to explore unified representations that better align heterogeneous modalities in a shared embedding space. We believe our benchmark can serve as a solid testbed for developing and evaluating such future methods.


% \subsection*{Weakness 2}
% Thank you for your valuable comment. We agree that the current title may be misleading, and we will revise it in the final version so that it more accurately reflects the paper’s focus on retrieval and its relationship to reasoning.

% \subsection*{Weakness 3}
% Thank you for your careful comment. We agree that the current description of \textbf{single-modality} and \textbf{cross-modality} can be confusing, and we will clarify this in the revised version: \textbf{single-modality} denotes retrieval when both the query and the database are restricted to a single data type (e.g., only videos), whereas \textbf{cross-modality} denotes retrieval from a mixed pool of images, videos, and documents.

% Regarding the fairness concern, we have conducted an additional experiment (not included in the current submission). For each modality, we first keep all ground-truth items in the pool. We then complete the pool by uniformly sampling additional items from each modality so that the proportions of image / video / document items match those in the full-size cross-modality setting, resulting in a mixed (image+video+document) retrieval pool \textbf{with the same total number of items as the corresponding single-modality pool}.

% These results indicate that even with an identical retrieval pool size, cross-modality retrieval remains substantially more difficult. Therefore, our conclusion that cross-modality is more challenging is not merely due to a smaller retrieval pool. We will clarify the definitions in Sec. 4.2/Line 294, update the text around Table 2 accordingly, and include these results in the appendix of the camera-ready version.


% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=\linewidth]{iclr2026/fig/reviewer93AH_weak3.pdf}
%     \caption{\textbf{pool size verification}}
%     \label{fig:poolsize}
% \end{figure}

% \subsection*{Weakness 4}
% visrag: 45.38/54.62/58.37

% \subsection*{Question 1}
% We thank the reviewer for this helpful suggestion. In the revised manuscript, we will clarify the distinction between page/frame-level and item-level at line 262 to avoid any ambiguity.

% \subsection*{Question 2}
% The results in Table 3 are obtained using the E5-V retrieval system. We will clarify this in the revised manuscript by explicitly specifying “E5-V” in the table caption.

% \subsection*{Question 3}
% Thank you for the suggestion. The overall performance across all tasks corresponding to Tables 4 and 5 is already reported in the “Overall” columns of Tables 2 and 3, respectively.

% \subsection*{Question 4}
% The primary contribution of this work is to construct and systematically analyze a large-scale cross-modal benchmark that reveals the limitations of existing models in realistic image–video–document retrieval scenarios, rather than to introduce a new retrieval algorithm. Consequently, within the scope and space of this paper, we focus on providing clear and representative baseline results instead of pursuing methodological innovations. We sincerely appreciate your specific suggestions, and in future work we plan to systematically explore agentic retrieval, query rewriting, and retrieval-database (key) augmentation techniques on top of this benchmark to better address this real-world task.

\section*{Reviewer 93AH (4)}
We are encouraged by your recognition of \textbf{our benchmark as a novel and challenging cross-modal setting with fine-grained evaluations.}
We will address your concern and answer your questions below.


\textbf{W1.~Scope of Contribution.}
Our goal is to introduce a benchmark—not a new retrieval method.  
(1) Sec.~5 shows that MultiHaystack uniquely exposes modality-mismatch, temporal misalignment, and fine-grained grounding failures across images, videos, and documents—failure modes that cannot be diagnosed without a unified, large-scale cross-modal pool.  
(2) No prior benchmark reveals the drastic cross-modal degradation observed in Fig.~8 and App.~G, confirming that MultiHaystack captures a missing evaluation regime.  
(3) We have added a brief discussion on future directions (Sec.~6)  directly motivated by these findings.

\textbf{W2.~Title Clarity.}
(1) Although the benchmark evaluates evidence-grounded reasoning, our experiments show that retrieval is the dominant bottleneck.  
(2) We agree the title should reflect this emphasis and will revise it accordingly.

\textbf{W3.~Single vs Cross Modality.}
(1) \emph{Definition:} Single-modality restricts both query and pool to one modality; cross-modality retrieves from a mixed pool (Sec.~4.2).  
(2) \emph{Controlled verification:} We constructed mixed pools with the \emph{same size} as the single-modality pools. As shown in Fig.~7, cross-modal retrieval remains substantially harder across modalities and TOP-k settings.  
(3) This confirms the challenge stems from modality heterogeneity—embedding mismatch and semantic interference—not pool size.

\textbf{Q1.~Page/Frame vs Item Level.}
Page/frame-level refers to internal segmentation of long documents/videos; item-level treats the whole file as the retrieval unit.  
We have clarified this in the paper.

\textbf{Q2.~Retriever Used in Table~3.}
Table~3 reports results using the E5-V retriever; we have stated this explicitly in the caption.

\textbf{Q3.~Overall Metrics.}
Overall results corresponding to Tables~4 and~5 already appear in the “Overall’’ columns of Tables~2 and~3.  
We have cross-referenced these locations for clarity.

\textbf{W4 \& Q4.~Task-level Insights and Practical Improvements.}
(1) Sec.~4.4.1 and Tables~4–5 show systematic variation across six task types; App.~G further visualizes distinct error profiles (contextual, factual, metadata, statistical, temporal, and layout-aware tasks).  
(2) These patterns suggest concrete remedies: entity-aware query rewriting, retrieval-key augmentation for numerical/structured content, time-anchored representations for videos, OCR/structure-aware encodings for layouts, and multi-step retrieve-then-reason cycles.  
(3) Our preliminary tests support this: in the E5-V–based cross-modal setting, RAG with a rewrite stage (+2.8\%), VisRAG (–7.7\%), and an agentic RAG system, MMsearch (+4.7\%), offer only modest improvements, while still falling well short of the single-modality upper bound (+9.7\%).
This validates our claim that the benchmark provides actionable insights while the tasks remain genuinely challenging.


\section*{Reviewer cRtU (8)}
We thank you for highlighting the strength of \textbf{our presentation, the comprehensiveness of our experiments, and the value of introducing a long-context tri-modal benchmark.}
We will address your concern and answer your questions below.

Following your suggestion, we evaluated the newer models InternVL-3.5 and Qwen2.5-VL, and both remain well below their single-modality upper bounds once retrieval is involved, confirming that even the latest models show the same limitations.
These results have been added to the revision (App. F3).



\begin{table*}[!ht]
  \centering
\caption{\textbf{VQA performance.} Each model answers questions using top-5 items retrieved from cross-modality inputs; {\color{gray}gray} numbers show single-modality Recall@5 for reference.}
  \resizebox{0.8\textwidth}{!}{%
    \setlength{\tabcolsep}{6pt}%
    \renewcommand{\arraystretch}{1.0}%
    \begin{tabular}{l c c c c}
      \toprule
      \textbf{Model} & \textbf{Video} & \textbf{Image} & \textbf{Document} & \textbf{Overall} \\
      \midrule

      InternVL-3.5 
      & 20.95 {\color{gray}\scriptsize(26.67)} 
      & 30.95 {\color{gray}\scriptsize(39.72)} 
      & 51.20 {\color{gray}\scriptsize(54.55)} 
      & 35.21 {\color{gray}\scriptsize(42.03)} \\

      Qwen2.5-VL  
      & 19.05 {\color{gray}\scriptsize(21.90)} 
      & 22.17 {\color{gray}\scriptsize(28.41)} 
      & 31.10 {\color{gray}\scriptsize(34.45)} 
      & 24.23 {\color{gray}\scriptsize(29.18)} \\
      
      \bottomrule
    \end{tabular}%
  }
\end{table*}




% \subsection{Weakness 1}
% Yes. As stated in Section 3.3 \textbf{MultiHaystack Construction}, Stage 1 *Data Collection* (lines 212–215), the raw multimodal data used in our benchmark (videos, images, and documents) are collected by integrating samples from several existing public benchmarks.

% However, we would like to emphasize that we \textbf{only use these existing benchmarks as sources of raw data}, and we \textbf{do not reuse their original task definitions or evaluation settings}. The tasks evaluated in our benchmark are fundamentally different from those in the source benchmarks in terms of both task formulation and evaluation focus. To construct a benchmark that aligns with our research goals and maintains high quality and appropriate difficulty, we design new tasks on top of this raw data and apply a multi-stage, non-trivial data curation pipeline that performs filtering, recombination, and quality control. The full construction process and implementation details are described in Section 3.3 *MultiHaystack Construction* of the paper.

% \subsection*{Weakness 2}
% In this paper, we do comprehensive analysis to highlight the need for retrieval-aware reasoning and modality-agnostic architectures.

% \subsection*{Question 1}
% Thank you for your question. Our retrieval corpus consists of three cross-modal types of files: videos, images, and documents, with a total of 45,260 files. More detailed statistics for each modality are provided in the “Data Profile” subsection of Section 3.3 “MultiHaystack Construction” (lines 253–254) in the paper.

% \subsection*{Question 2}
% \textbf{On the types of retrieved information.}

% Our system retrieves \textbf{multi-modal} information consisting of \textbf{videos, images, and textual documents}. These three modalities are stored in a unified index: for each query, we retrieve the most relevant multi-modal entries from this index and provide them to the model as contextual input.

% \textbf{On how we ensure that the retrieved context is useful.}

% This is empirically validated in our ablation study in Appendix Table F.1: when the model answers based only on the raw query, without using any retrieved context, its accuracy is extremely low and almost close to zero. In contrast, as shown in Table 3 in the main paper, when the model uses the top-5 retrieved items as context, its performance improves substantially.

% This large performance gap clearly indicates that the retrieved context is \textbf{both necessary and beneficial} for the model’s reasoning, thereby providing empirical evidence that the retrieved context is indeed useful.

% \subsection*{Question 3}
% Yes.


% \subsection*{Question 4}
% ...


\section*{Reviewer nMyE (4)}
We appreciate your acknowledgment that \textbf{MultiHaystack is the first large-scale benchmark for realistic cross-modal retrieval and your recognition of our comprehensive model evaluations.}
We will address your concern and answer your questions below.

\textbf{W1.~Clarity of Presentation.}
We appreciate the reviewer’s concern. However, other reviewers found the presentation clear and well structured, and Sec.~3.3 together with Fig.~4 already outlines the pipeline stage by stage. If any specific part remains unclear, we are happy to clarify it further.


\textbf{W2.~Use of Existing Benchmarks.}
As stated in Sec.~3.3, prior datasets are used only as \emph{raw multimodal files}; no tasks, labels, or evaluations are reused.  
MultiHaystack introduces a new evaluation regime:  
a unified cross-modal pool (videos+images+documents), human-validated and uniquely supported QA, removal of questions answerable without evidence, and controlled cross-modal distractor construction.  
This multimodal needle-in-haystack setting does not exist in any source benchmark, making MultiHaystack a \textbf{new benchmark rather than a combination of prior tasks}.  


\textbf{W3.~Significant Experimental Findings.}
A key scientific finding enabled only by MultiHaystack is the large and consistent gap between \emph{“gold evidence given’’} and \emph{“retrieval required’’} across all models.  
Once evidence is provided, reasoning is strong; the dominant bottleneck is cross-modal retrieval—driven by embedding mismatch and semantic interference.  
This divergence does \emph{not} appear in single-modality or small-pool benchmarks, highlighting that MultiHaystack uncovers failure modes not observable in prior datasets.
Thus, the benchmark reveals a previously undocumented failure mode in modern MLLMs.

\textbf{Q1.~Composition of the Retrieval Corpus.}
The retrieval corpus contains 45{,}260 items (videos, images, documents).  
Detailed statistics are reported in Sec.~3.3 and App.~A.

\textbf{Q2.~Retrieved Information and Usefulness.}
Retrieved evidence includes videos, images, and documents from a unified index.  
Usefulness is guaranteed by construction: each QA pair is grounded to a \emph{unique} supporting page/frame/item, and the single-supported-answer filter ensures that this item contains all necessary evidence.  
Empirically, Appendix Table~F.1 shows near-zero accuracy without retrieved context, while Table~3 shows large gains with retrieved items.

\textbf{Q3.~Ground-truth Retrieval.}
Yes. Each QA pair specifies the ID of its unique supporting item.

\textbf{Q4.~Bounding Boxes.}
The benchmark does not use bounding boxes.  
Ground truth is provided at the page/frame/item level, as the task evaluates item-level retrieval and evidence-grounded reasoning rather than spatial localization.

==> table/up_bound.tex <==
\begin{table*}[!ht]
\centering
\caption{\textbf{Upper-bound analysis for VQA models.} We estimate ceilings under three evidence regimes: G@1 (Gold in Top-1)—the ground-truth positive item is given as the only context; G@5 (Gold in Top-5)—the positive item is inserted at a random position among five candidates; and R@5 (Recall@5)—the top-5 items returned by the E5-V retriever are provided as context. Reported scores reflect VQA performance conditioned on each regime. }
\label{tab:up_bound}
\resizebox{\textwidth}{!}{%
\setlength{\tabcolsep}{6pt}%
\renewcommand{\arraystretch}{0.9}%
\begin{tabular}{l ccc ccc ccc ccc}
\toprule
\multirow{2}{*}{\textbf{Model}} &
\multicolumn{3}{c}{\textbf{Video}} &
\multicolumn{3}{c}{\textbf{Image}} &
\multicolumn{3}{c}{\textbf{Document}} &
\multicolumn{3}{c}{\textbf{Overall}} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}
& \textbf{G@1} & \textbf{G@5} & \textbf{R@5}
& \textbf{G@1} & \textbf{G@5} & \textbf{R@5}
& \textbf{G@1} & \textbf{G@5} & \textbf{R@5}
& \textbf{G@1} & \textbf{G@5} & \textbf{R@5} \\
    \midrule
Ola        & 59.05 & 48.57 & 14.29 & 46.42 & 38.11 & 20.09 & 59.33 & 51.20 & 36.36 & 51.81 & 43.24 & 23.83 \\
InternVL-3 &  63.81   & 55.24    &  17.14   &  48.50   & 40.42    & 29.33    &  64.11   &  57.89   &  49.28   & 55.02   &  47.39   & 33.29    \\
Qwen2-VL    & 54.29 &  45.71 & 16.19 & 37.18 & 30.25 &  16.86 & 49.76 & 42.58 & 19.62 & 43.11 & 35.88 & 17.54 \\
Gemini-2.5-Flash  & 85.71 & 81.90 & 52.38 & 69.52 &  47.34 & 35.10 &  79.90 & 74.16 & 56.94 & 74.70 & 59.71 & 43.64 \\
GPT-5  & \textbf{89.52} &  \textbf{85.71} & \textbf{60.00} &  \textbf{75.75} &  \textbf{59.82} & \textbf{43.19} & \textbf{87.08} & \textbf{78.47}  & \textbf{64.11}  & \textbf{80.86} & \textbf{68.67} & \textbf{51.41} \\
\bottomrule
\end{tabular}}
\end{table*}

==> table/vqa_different_modality.tex <==
\begin{table*}[!ht]
  \centering
   \caption{\textbf{Performance Comparison.} Evaluation of the VQA performance for representative multi-modal models across three distinct input modalities.}
  \label{tab:vqa_different_modality}
  \resizebox{0.65\textwidth}{!}{%
    \setlength{\tabcolsep}{6pt}%
    \renewcommand{\arraystretch}{0.9}%
    \begin{tabular}{l c c c c}
      \toprule
      \textbf{Model}           & \textbf{Video} & \textbf{Image} & \textbf{Document} & \textbf{Overall} \\
      \midrule
      Ola  ~\cite{liu2025ola}        & 14.29 & 20.09 & 36.36  &  23.83  \\
      InternVL-3  ~\cite{Zhu2025InternVL3EA} & 17.14 & 29.33 & 49.28 & 33.20 \\
      Qwen2-VL  ~\cite{Qwen2VL}   & 16.19 & 16.86 & 19.62 & 17.54 \\
      Gemini-2.5-Flash   ~\cite{google2024gemini}    & 52.38 & 35.10 & 56.94 & 43.64 \\
      GPT-5  ~\cite{openai2025-gpt5}     & \textbf{60.00} & \textbf{43.19} & \textbf{64.11} & \textbf{51.41} \\
      \bottomrule
    \end{tabular}%
  }
\end{table*}
